The Physical Meaning of Time-Delayed Collection Field Transients from Disordered Devices

Charge carrier mobility and recombination determine the performance of many opto-electronic devices such as solar cells, sensors and light-emitting diodes. Understanding how these parameters change as a function of material choice, charge carrier density and device geometry is essential for developing the next generation of devices. The Time-Delayed-Collection-Field technique (TDCF) is becoming a widely used method to measure both recombination and carrier transport with values derived from this method being widely reported for many material systems. However, most novel materials are highly disordered with a high density of trap states and standard TDCF-theory neglects the influence of these states. In this work we examine how reliable TDCF can be as a measurement technique when the device contains significant energetic disorder. We identify regimes where the results can be relied upon and where the results should be taken with more caution. Finally, we provide simple and easy to use experimental tests to help the experimentalist decide if the physical processes are dominated by trap states.

==> paper/mobility_main.tex <==
\subsection{Main figures mobility}

TDCF mobility determination works well for devices with free charge carriers only (few traps).

Insight into charge carrier trapping in the device. 

Extract times to calculate mobility from $\Theta(t)$ and $j_{\mathrm{trap}}$.

Show that they have the same trend as the mobility extracted from linear fits of the photo current. The predicted mobility does not correspond to the real (correct) mobility.

\begin{figure}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width = \textwidth]{methods/bilder/mu_fit.png}
        \caption{fit method}
        \label{fig:mobility_asym_fitmax}
    \end{subfigure}
    \hspace{\xvert\textwidth}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
         \includegraphics[width = \textwidth]{methods/bilder/mu_integral.png}
        \caption{integration method}
        \label{fig:mobility_asym_intmax}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width = \textwidth]{tdcf_mobility/bilder/mufit_mumax_error_matrix.png}
        \caption{Comparison of higher charge carrier mobility with determined mobility by the fit method}
        \label{fig:mobility_asym_fitmax}
    \end{subfigure}
    \hspace{\xvert\textwidth}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
         \includegraphics[width = \textwidth]{tdcf_mobility/bilder/mui_mumax_error_matrix.png}
        \caption{Comparison of higher charge carrier mobility with determined mobility by the integration method}
        \label{fig:mobility_asym_intmax}
    \end{subfigure}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width = \textwidth]{tdcf_mobility/bilder/mufit_mumin_error_matrix.png}
        \caption{Comparison of lower charge carrier mobility with determined mobility by the fit method.}
        \label{fig:mobility_asym_fitmin}
    \end{subfigure}
    \hspace{\xvert\textwidth}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
         \includegraphics[width = \textwidth]{tdcf_mobility/bilder/mui_mumin_error_matrix.png}
        \caption{Comparison of lower charge carrier mobility with determined mobility by the integration method.}
        \label{fig:mobility_asym_intmin}
    \end{subfigure}
    \caption{Error matrices for asymmetric input mobilities in the range of $\mux{inp} = 10^{-10}~\text{to}~10^{-4}\unit{m^{2}V^{-1}s^{-1}}$ without trap states. Compared are the extracted mobilities with both methods to minimum and maximum free charge carrier mobility for random generated hole and electron mobility pairs.}
    \label{fig:mobility_asym}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width = \textwidth]{paper/bilder/mufit_mufree_withoutrc_error_matrix.png}
        \caption{Mobility determination with fit-method for the case without trap states.}
    \end{subfigure}
    \hspace{\xvert\textwidth}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width = \textwidth]{paper/bilder/mufit_mufree_error_matrix.png}
        \caption{Mobility determination with fit-method for the case with trap states.}
        \label{fig:mobility_nextract_25}
    \end{subfigure}
    \caption{Comparison of determined mobility by linear photo-current decay for the case with and without trap states. the deviation from the true mobility for high input mobilities is due to the RC-time of the device (see SI) }
    \label{fig:mobility_trap_mu_trap}
\end{figure}

\clearpage
Tests to see if trap states play a role in a given device. (suppossed to be quick and combined with a-priory knowledge, if not sufficient one has to use photo-voltage measurements, space-charge-limited measurements, thermally stimulated current measurements or impedance-spectroscopy experiments)

Show that trap state density can have a severe impact on current transients especially at long extraction times. Idea similar to \cite{Hanfland2013CELIV}.

Show that 
\begin{equation}\label{eq:mob_ratio}
    \mathrm{ratio} = \frac{\int\limits_{t_\mathrm{1/2}}^{t_\mathrm{end}} j(t) \mathrm{d}t}{\int\limits_{0}^{t_\mathrm{end}} j(t) \mathrm{d}t}
\end{equation} 
is a good indicator for the presence of high trap state densities.

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{paper/bilder/fig3.png}
    \caption{ Comparison of current transients for different trap state densities and voltages. High trap state densities show a long lasting high extraction current.}
    \label{fig:mobility_ratio_vgl_trap}
\end{figure}

\clearpage
Show that charge carrier extraction becomes intensity dependent for high trap state densities (because at high intensities, deep traps are filled and more charge carriers reside in shallow traps and can get extracted more easily)

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width = \textwidth]{tdcf_mobility/bilder/2022_06_13_mob_symm_nextract_5e19.png}
        \caption{Trap state density $n_\mathrm{trap} = 5\cdot10^{19}\unit{m^{-3}}$}
        \label{fig:mobility_nextract_19}
    \end{subfigure}
    \hspace{\xvert\textwidth}
    \begin{subfigure}[t]{0.4\linewidth}
        \centering
        \includegraphics[width = \textwidth]{tdcf_mobility/bilder/2022_06_13_mob_symm_nextract_5e25.png}
        \caption{Trap state density $n_\mathrm{trap} = 5\cdot10^{25}\unit{m^{-3}}$.}
        \label{fig:mobility_nextract_25}
    \end{subfigure}
    \caption{Simulated maps of extracted charge carrier density during steady state JV-measurements depending on applied bias and illumination density.}
    \label{fig:mobility_nextract}
\end{figure}

\clearpage
Band diagram to illustrate: for low Ntrap free charges get extracted easily, after that only deep trap states / for high Ntrap Nfree $\approx$ Ntrap and shallow traps can get extracted easily

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{tdcf_mobility/bilder/2022_06_24_mob_symm_nextract_bands_4.44suns_-0.15V.png}
    \caption{Free charge carrier density and trapped charge carrier density with the according band diagrams. The two cases depicted are data points in \cref{fig:mobility_nextract_19} and \cref{fig:mobility_nextract_25} respectively at around $I = 4.5\unit{suns}$ and $V = -0.15\unit{V}$.}
    \label{fig:mobility_band}
\end{figure}

==> paper/recombination_main.tex <==
\subsection{Main figures recombination}

Drift diffusion simulation to see recombination rate dependency on charge carrier density  internal in the device by combining the time transients.

\clearpage
See usual case without high initial rec rates in SI. kniepert

dn/dt  and delay time dependent recombination order from TDCF simulations for the case with dominating charge carrier extraction

Comparison of Rsurf(n) with TDCF-data for one light intensity

dn/dt  and delay time dependent recombination order from TDCF simulations for the case with dominating relaxation of charge carriers into trap states

Comparison of Rsurf(n) with TDCF-data for one light intensity

\begin{figure*}
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \includegraphics[width = \textwidth]{tdcf_recomb/bilder/tdcf_tdcf_1.0e-07_1.0e-07_5.0e+25_1.0e-20_R(n)_5.0_shift_1.26e+23_n_and_p_surf.png}
        \caption{Comparison of TDCF-data with R(n): R is surface-recombination $R_{\mathrm{surf}}$.}
        \label{fig:tdcf_r(n)_extract}
    \end{subfigure}
    \hspace{\xvert\textwidth}
    \begin{subfigure}[t]{0.49\linewidth}
        \includegraphics[width = \textwidth]{tdcf_recomb/bilder/tdcf_tdcf_1.0e-07_1.0e-07_5.0e+25_1.0e+25_R(n)_0.1_shift_1.93e+23.png}
        \caption{Comparison of TDCF-data with R(n): R is Shockley-Read-Hall recombination rate $R_{\mathrm{SRH}}$.}
        \label{fig:tdcf_trap_r(n)}
    \end{subfigure}
    \caption{Recombination in TDCF-experiments averaged rec. rate from TDCF and actual rec. rate inside the device for domainating Rsurf and dominating Rsrh.}
    \label{fig:tdcf_trap}
\end{figure*}

\input{tdcf_recomb/table_tdcf_rec_surf}
\input{tdcf_recomb/table_tdcf_rec_exptrap}

In both cases the high initial recombination orders can be explained as a relaxation of the recombination order due to quickly decreasing free charge carrier densities (either by thermalization or extraction). To distinguish the cause of the relaxation, the delay time dependent recombination order is an important tool. Recombination orders of $\delta \leq 2$ at long times can be attributed to the recombination of free charge carriers. Recombination orders of $\delta(\td) = 1$ point towards dominating surface recombination. For cases with dominating traps a $\delta = 1.4$ for exponential distribution of trap states was derived in literature \cite{Hofacker_Neher2017dispersiverecomb}.


==> paper/table_rec_sim_reference_kniepert.tex <==
\begin{table}[H]
    \caption[Simulation parameters \textbf{Case 0}: recombination reference system PM6:Y6 after \cite{Kniepert2019Chargeextraction}]{\label{tab:rec_reference_kniepert}Simulation parameters \textbf{Case 0}: recombination reference system PM6:Y6 after \cite{Kniepert2019Chargeextraction}}
    \centering
    \begin{tabular}{ll}
	    \hline\hline
	    Parameter & Value\\
	     & \\\hline
		  Active layer & PM6:Y6 $d = 10^{-7}\unit{m}$\\ \hline
		  Effective bandgap & $E_\mathrm{g} = 1.25\unit{eV}$\\ \hline
		  Cell area & $A = 0.5\cdot 0.5\unit{mm^2}$\\ \hline
		  Input mobility & $\mu_\mathrm{e} = \mu_\mathrm{h} = 10^{-7}\unit{\frac{m^2}{Vs}}$\\ \hline
		  Effective charge carrier density & $n_\mathrm{eff} =5\cdot 10^{25}\unit{m^{-3}}$\\ \hline
		  Free-to-free recombination rate & $k_2 = 10^{-17}\unit{m^{3}s^{-1}}$\\ \hline
		  Laser intensity & $I = 0.1 ~\text{to}~ 5.0 \unit{\frac{\mu J}{cm^2}}$\\\hline
		  Pre-bias & $\vpre = 0.7\unit{V}$\\ \hline
		  Collection-bias & $\vcol = -2.5\unit{V}$\\ \hline
		  Delay time & $\td = 5\unit{ns}~\text{to}~5\cdot 10^{-7}\unit{s}$\\
		 \hline \hline
	\end{tabular}
\end{table}
